Towards the routine use of subdominant harmonics in gravitational-wave inference: re-analysis of GW190412 with generation X waveform models

We re-analyse the gravitational-wave event GW190412 with state-of-the-art phenomenological waveform models. This event, which has been associated with a black hole merger, is interesting due to the significant contribution from subdominant harmonics. We use both frequency-domain and time-domain waveform models. The PhenomX waveform models constitute the fourth generation of frequency-domain phenomenological waveforms for black hole binary coalescence; they have more recently been complemented by the time-domain PhenomT models, which open up new strategies to model precession and eccentricity, and to perform tests of general relativity with the phenomenological waveforms approach. Both PhenomX and PhenomT have been constructed with similar techniques and accuracy goals, and due to their computational efficiency this "generation X" model family allows the routine use of subdominant spherical harmonics in Bayesian inference. We show the good agreement between these and other state-of-the-art waveform models for GW190412, and discuss the improvements over the previous generation of phenomenological waveform models. We also discuss practical aspects of Bayesian inference such as run convergence, variations of sampling parameters, and computational cost.

==> Preamble.tex <==
%auto-ignore

\makeatletter

%% Smaller space between section number and name
\def\@seccntformat#1{\csname the#1\endcsname.~}%

%% Smaller space between preceding text and new section headings
\def\section{%
  \@startsection {section}
  {1} {\z@} {0.55cm \@plus1ex \@minus .02ex}%
    {0.225cm} { \normalfont\bfseries \centering}%
}%
\def\subsection{%
  \@startsection {subsection}
  {2} {\z@ } {0.45cm \@plus 0.8ex \@minus 0.2ex}%
  {0.1125cm}{\normalfont \bfseries \centering }}
\def\subsubsection{%
  \@startsection {subsubsection}
  {3} {\z@ } {0.4cm \@plus 0.6ex \@minus 0.1ex}%
  {0.075cm}{\normalfont \it \centering }}

%% Headers and footers
\newcommand{\surnames}[1]{\def\@surnamelist{#1}\relax}
\surnames{\ }
\ifx \@shorttitle \@empty
  % \def\@oddhead{\small \MakeUppercase{\@title} \hfill}
  % Do nothing
\else
  \def\@oddhead{\small \MakeUppercase{\@shorttitle} \hfill}
\fi
\ifx \@surnamelist \@empty
  % Do nothing
\else
  \def\@evenhead{\small \MakeUppercase{\@surnamelist} \hfill}
\fi
\def\@oddfoot{\reset@font\hfil\thepage\hfil}%
\def\@evenfoot{\reset@font\hfil\thepage\hfil}%
\g@addto@macro\maketitle{\global\@specialpagetrue\gdef\@specialstyle{plain}}

%% Less hyphenation
\hyphenpenalty=1000  % Default: 50
%\tolerance=9000      % Default: 9999

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package and nice colors

%% The following conflicts with \texorpdfstring in section headers
% %% First, patch a bug from revtex4 to allow use of \nameref
% \usepackage{xpatch}% http://ctan.org/pkg/xpatch
% \makeatletter
% \xpatchcmd{\@ssect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>*
% \xpatchcmd{\@sect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>
% \makeatother

\definecolor{dodgerblue}{rgb}{0.12, 0.56, 1.0}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{alizarincrimson}{rgb}{0.82, 0.1, 0.26}
\definecolor{mediumpurple}{rgb}{0.58, 0.44, 0.86}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}
\definecolor{my_gray}{rgb}{0,0,0}
\definecolor{uniwienblue}{HTML}{006699}
\definecolor{walesred}{HTML}{ff0038}
\definecolor{myorange}{HTML}{FF6C0C}
\definecolor{ferngreen}{HTML}{009246}
\definecolor{scarletred}{HTML}{CD212A}

\usepackage[colorlinks, plainpages=false,
hyperfigures=true]{hyperref}
% \usepackage[pagebackref=true, colorlinks, plainpages=false,
% hyperfigures=true]{hyperref}
% \renewcommand*{\backref}[1]{}
% \renewcommand*{\backrefalt}[4]{%
%   \ifcase #1 \or (Cited on p.~#2.) \else %
%   (Cited on pp.~#2.) \fi %
% }
\hypersetup{linkcolor=dodgerblue}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=dodgerblue}
\hypersetup{setpagesize=false}
% \hypersetup{unicode} % Clashes with '\G' command defined in Macros
\hypersetup{pdfborder=0 0 0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatother

%\numberwithin{equation}{section}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

